Actor-Critic based Improper Reinforcement Learning

We consider an improper reinforcement learning setting where a learner is given $M$ base controllers for an unknown Markov decision process, and wishes to combine them optimally to produce a potentially new controller that can outperform each of the base ones. This can be useful in tuning across controllers, learnt possibly in mismatched or simulated environments, to obtain a good controller for a given target environment with relatively few trials. Towards this, we propose two algorithms: (1) a Policy Gradient-based approach; and (2) an algorithm that can switch between a simple Actor-Critic (AC) based scheme and a Natural Actor-Critic (NAC) scheme depending on the available information. Both algorithms operate over a class of improper mixtures of the given controllers. For the first case, we derive convergence rate guarantees assuming access to a gradient oracle. For the AC-based approach we provide convergence rate guarantees to a stationary point in the basic AC case and to a global optimum in the NAC case. Numerical results on (i) the standard control theoretic benchmark of stabilizing an cartpole; and (ii) a constrained queueing task show that our improper policy optimization algorithm can stabilize the system even when the base policies at its disposal are unstable.

==> bandits_over_bandits.tex <==
\subsection{Bandit over Bandits}\label{sec:bandit over bandit}
%Here, $S=1$, and a finite number of actions $\abs{\cA} =A$. 
Note once again that each controller in this case, is a probability distribution over the $A$ arms of the bandit. We consider the scenario where the agent at each time $t\geq 1$, has to choose a probability distribution $K_{m_t}$ from a set of $M$ probability distributions over actions $\cA$. She then plays an action $a_t\sim K_{m_t}$. This is different from the standard MABs because the learner cannot choose the actions directly, instead chooses from a \emph{given} set of controllers, to play actions. 
% Again, the goal of the learner is to find the best controller in the \enquote{convex hull} of the given set of $M$ controllers, i.e., find
% \begin{equation}
%     \pi^* =\argmax\limits_{\pi\in \cP([M])} V^\pi.
% \end{equation}
%\[\pi^* =\argmax\limits_{\pi\in \cP([M])} V^\pi. \]
Note the $V$ function has no argument as $S=1$.
Let $\mu\in [0,1]^A$ be the mean vector of the arms $\cA$. The value function for any given mixture $\pi\in \cP([M])$, 
\begin{align}\label{eq:bandits-value function}
    V^\pi &\bydef \expect{\sum\limits_{t=0}^\infty \gamma^tr_t\given \pi } = \sum\limits_{t=0}^\infty \gamma^t\expect{r_t\given \pi}
    =\sum\limits_{t=0}^\infty \gamma^t\sum\limits_{a\in \cA}\sm  \pi(m)K_m(a)\mu_a. \nonumber\\
    &= \frac{1}{1-\gamma} \sm \pi_m \mu\transpose K_m = \frac{1}{1-\gamma} \sm \pi_m \mathfrak{r}^\mu_m. 
\end{align}
where the interpretation of $\kr_m^\mu$ is that it is the mean reward one obtains if the controller $m$ is chosen at any round $t$. 
 Since $V^{\pi}$ is linear in $\pi$, the maximum is attained at one of the base controllers $\pi^*$ puts mass 1 on $m^*$ where
 $m^*:= \argmax\limits_{m\in [M]} V^{K_m},$
and $V^{K_m}$ is the value obtained using $K_m$ for all time. In the sequel, we assume $\Delta_i\bydef \mathfrak{r}^\mu_{m^*}-\mathfrak{r}^\mu_i>0$.
%For this special case we show two results.

\subsection{Perfect Gradient Knowledge}
With access to the exact value gradient at each step, we 
%follow SPG \ref{alg:mainPolicyGradMDP} (sans the state update step of course). We 
have the following result.
\begin{restatable}{theorem}{convergencebandits}\label{thm:convergence for bandit}
With $\eta=\frac{2(1-\gamma)}{5}$ and with $\theta^{(1)}_m=1/M$ for all $m\in [M]$, with the availability for true gradient, we have $\forall t\geq 1$,
\[V^{\pi^*}-V^{\pi_{\theta_t}} \leq \frac{5}{1-\gamma} \frac{M^2}{t}.\]
\end{restatable}
Also, defining regret for a time horizon of $T$ rounds as %for the MAB setups as
\begin{equation}\label{eq:regret definition MAB}
    \mathcal{R}(T):= \sum\limits_{t=1}^T V^{\pi^*} - V^{\pi_{\theta_t}},
\end{equation}
we show as a corollary to Thm.~\ref{thm:convergence for bandit} that,
\begin{corollary}\label{cor:regret true gradient MAB}
\[\mathcal{R}(T)\leq \min\left\{ \frac{5M^2}{1-\gamma}{\color{blue}\log T}, \sqrt{\frac{5}{1-\gamma}}M{\color{blue}\sqrt{T}} \right\}. \]
\end{corollary}
\begin{proof}[Proof sketch of Theorem \ref{thm:convergence for bandit}]
The proof flows along similar lines as that of Theorem 3 in \cite{Mei2020}. First we establish that $V^\pi$ is $\frac{5}{2(1-\gamma)}$-smooth. Since smoothness alone does not guarantee convergence and  convergence rates, we establish a lower bound on the norm of the gradient of the value function at every step $t$ as below (these type of inequalities are called {\L}ojaseiwicz inequalities \cite{lojasiewicz1963equations})
\begin{lemma}\label{lemma:nonuniform lojaseiwicz MAB}[Lower bound on norm of gradient]
\[\norm{\frac{\partial V^{\pi_\theta}}{\partial \theta}}_2 \geq \pi_{\theta_{m^*}} \left(V^{\pi^*}-V^{\pi_{\theta}}\right). \]
\end{lemma}
Intuitively, this ``gradient domination" helps the algorithm to not get stuck in a local maxima. We refer the reader to section \ref{appendix:proofs for MABs} for all the proofs for this section.
\end{proof}
\subsection{Convergence with Noisy Gradient Estimates}
When value gradients are unavailable, we follow a direct policy gradient algorithm instead of softmax projection) (see Algorithm \ref{alg:ProjectionFreePolicyGradient}). At each round $t\geq 1$, the learning rate for $\eta$ is chosen asynchronously for each controller $m$, to be $\alpha \pi_t(m)^2$, to ensure that we remain inside the simplex, for some $\alpha \in (0,1)$. To justify its name as a policy gradient algorithm, observe that in order to minimize regret, we need to solve the following optimization problem:
\[\min\limits_{\pi\in \cP([M])} \sm \pi(m)(\kr_\mu(m^*)- \kr_\mu(m)). \]
A direct gradient with respect to the parameters $\pi(m)$ gives us a rule for the policy gradient algorithm. The other changes in the update step (eq \ref{algstep:update noisy gradient}), stem from the fact that true means of the arms are unavailable and importance sampling.

\setlength{\textfloatsep}{10pt}
\begin{wrapfigure}{L}{0.55\textwidth}
    \begin{minipage}{0.55\textwidth}
      \begin{algorithm}[H]
         \caption{PG for Bandit-over-bandits with Direct Parameterization}
         \label{alg:ProjectionFreePolicyGradient}
\begin{algorithmic}
   \STATE {\bfseries Input:} learning rate $\eta\in (0,1)$
   %\REPEAT
   \STATE Initialize each $\pi_1(m)=\frac{1}{M}$, for all $m\in [M]$.
   \FOR{$t=1$ {\bfseries to} $T$}
   \STATE $m_*(t)\leftarrow \argmax\limits_{m\in [M]} \pi_t(m)$
   \STATE Choose controller $m_t\sim \pi_t$.
   \STATE Play action $a_t \sim K_{m_t}$.
   %\IF{$x_i > x_{i+1}$}
   \STATE Receive reward  $R_{m_t}$ by pulling arm $a_t$.
   \STATE Update $\forall m\in [M], m\neq m_*(t): $ 
   \begin{equation}\label{algstep:update noisy gradient}
   \pi_{t+1}(m) = \pi_t(m) + \eta\left(\frac{R_{m}\ind_{m}}{\pi_t(m)} - \frac{R_{m_*(t)}\ind_{m_*(t)}}{\pi_t(m_*(t))}\right)    
   \end{equation}
   \STATE Set $\pi_{t+1}(m_*(t)) = 1- \sum\limits_{m\neq m_*(t)}\pi_{t+1}(m)$.
   %\ENDIF
   \ENDFOR
   %\UNTIL{$noChange$ is $true$}
\end{algorithmic}
      \end{algorithm}
      \vspace{-2cm}
    \end{minipage}
  \end{wrapfigure}


% \begin{algorithm}[tb]
%   \caption{Projection-free Policy Gradient (for MABs)}
%   \label{alg:ProjectionFreePolicyGradient}
% \begin{algorithmic}
%   \STATE {\bfseries Input:} learning rate $\eta\in (0,1)$
%   %\REPEAT
%   \STATE Initialize each $\pi_1(m)=\frac{1}{M}$, for all $m\in [M]$.
%   \FOR{$t=1$ {\bfseries to} $T$}
%   \STATE $m_*(t)\leftarrow \argmax\limits_{m\in [M]} \pi_t(m)$
%   \STATE Choose controller $m_t\sim \pi_t$.
%   \STATE Play action $a_t \sim K_{m_t}$.
%   %\IF{$x_i > x_{i+1}$}
%   \STATE Receive reward  $R_{m_t}$ by pulling arm $a_t$.
%   \STATE Update $\forall m\in [M], m\neq m_*(t): $ 
%   \begin{equation}\label{algstep:update noisy gradient}
%   \pi_{t+1}(m) = \pi_t(m) + \eta\left(\frac{R_{m}\ind_{m}}{\pi_t(m)} - \frac{R_{m_*(t)}\ind_{m_*(t)}}{\pi_t(m_*(t))}\right)    
%   \end{equation}
%   \STATE Set $\pi_{t+1}(m_*(t)) = 1- \sum\limits_{m\neq m_*(t)}\pi_{t+1}(m)$.
%   %\ENDIF
%   \ENDFOR
%   %\UNTIL{$noChange$ is $true$}
% \end{algorithmic}
% \end{algorithm}

We have the following result.
\begin{restatable}{theorem}{regretnoisyMAB}\label{thm:regret noisy gradient}
With value of $\alpha$ chosen to be less than $\frac{\Delta_{min}}{\mathfrak{r}^\mu_{m^*}-\Delta_{min}}$, $\left(\pi_t\right)$ is a Markov process, with $\pi_t(m^*)\to 1$ as $t\to \infty, a.s.$ Further the regret till any time $T$ is bounded as
\[\cR(T) \leq \frac{1}{1-\gamma}\sum\limits_{m\neq m^*} \frac{\Delta_m}{\alpha\Delta_{min}^2} \log T + C,\]
\end{restatable}
where $C\bydef \frac{1}{1-\gamma}\sum\limits_{t\geq 1}\mathbb{P}\left\{\pi_{t}(m^*(t)) \leq \frac{1}{2}\right\}<\infty$.

The proof follows similar lines as in \cite{Denisov2020RegretAO}.
Again we refer Appendix \ref{appendix:proofs for MABs} for the proof of this theorem. We make couple of remarks.

\begin{remark}\label{remark:relation between true and noisy grad}
The ``cost" of not knowing the true gradient seems to cause the dependence on $\Delta_{min}$ in the regret, as is not the case when true gradient is available (see Theorem \ref{thm:convergence for bandit} and Corollary \ref{cor:regret true gradient MAB}). The dependence on $\Delta_{min}$ as is well known from the work of \cite{LAI19854}, is unavoidable.
\end{remark}

\begin{remark}\label{remark:dependence on delta}
The dependence of $\alpha$  on $\Delta_{min}$ can be removed by a more sophisticated choice of learning rate, at the cost of an extra $\log T$ dependence on regret \cite{Denisov2020RegretAO}.  
\end{remark}

==> checklist_2021.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

% %%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}%\answerTODO{}
  \item Did you describe the limitations of your work?
    \answerYes{The assumptions made for showing our convergence results are discussed in Sec.~\ref{sec:theoretical-convergence-results}. The discussion following Theorem \ref{thm:convergence of policy gradient} covers the lack of theoretical understanding of the key constant $c$. Section \ref{subsec:theory-estimated-gradients} discusses the challenges involved in showing convergence rates for general MDPs. }%\answerTODO{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{Please see Sec.~\ref{sec:conclusion-and-discussion} for a  discussion.}%\answerTODO{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}%\answerTODO{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}%\answerTODO{}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{Due to paucity of space, we have moved all the proofs to the supplementary material, which we have submitted along with the paper. However, the proofs within the Appendix are themselves \emph{\color{blue}complete} and require no additional material.}%answerTODO{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}%\answerTODO{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{We have provided all details of hyperparameters necessary to reproduce our results in Sec.~\ref{sec:simulation-details} of the Appendix}%\answerTODO{}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}%\answerTODO{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{Please check the section on Simulation Details.}%\answerTODO{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerNA{}%\answerTODO{}
  \item Did you mention the license of the assets?
    \answerNA{}%\answerTODO{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}%\answerTODO{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}%\answerTODO{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}%\answerTODO{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}%\answerTODO{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}%\answerTODO{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}%\answerTODO{}
\end{enumerate}

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> figures/fig_queueing_motivation.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        
% SYNTAX: \resizebox{width}{height}
\resizebox{9.50cm}{3.75cm}{

\begin{tikzpicture}[x=0.5pt,y=0.5pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,273); %set diagram left start at 0, and has height of 273

%Straight Lines [id:da09715700995858345] 
\draw [line width=1.5]    (81.8,155.36) -- (260.8,155.36) ;
%Straight Lines [id:da8887479227991981] 
\draw [line width=1.5]    (80.8,215.36) -- (260.8,216.36) ;
%Straight Lines [id:da6217209993953612] 
\draw    (61.8,185.36) -- (89.8,185.36) ;
\draw [shift={(91.8,185.36)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da875509031522369] 
\draw [line width=1.5]    (260.8,155.36) -- (260.8,216.36) ;
%Straight Lines [id:da37671038244024846] 
\draw    (180,45) -- (257.8,45) ;
\draw [shift={(260.8,45)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
\draw [shift={(177,45)}, rotate = 0] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da0678614898035077] 
\draw    (122.8,225) -- (257.8,225) ;
\draw [shift={(260.8,225)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
\draw [shift={(119.8,225)}, rotate = 0] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Shape: Circle [id:dp028275738414681006] 
\draw  [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=0.67 ] (365,142.18) .. controls (365,134) and (371.63,127.36) .. (379.82,127.36) .. controls (388,127.36) and (394.64,134) .. (394.64,142.18) .. controls (394.64,150.37) and (388,157) .. (379.82,157) .. controls (371.63,157) and (365,150.37) .. (365,142.18) -- cycle ;
%Curve Lines [id:da7202837492936005] 
\draw    (343.8,77.36) .. controls (279.45,122.9) and (302.33,173.34) .. (342.58,204.43) ;
\draw [shift={(343.8,205.36)}, rotate = 217.09] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da4678251099443136] 
\draw    (365,142.18) -- (288.45,89.5) ;
\draw [shift={(286.8,88.36)}, rotate = 394.53999999999996] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Axis 2D [id:dp8494447421977243] 
\draw [line width=1.5]  (472,195.73) -- (648.8,195.73)(489.68,64) -- (489.68,210.36) (641.8,190.73) -- (648.8,195.73) -- (641.8,200.73) (484.68,71) -- (489.68,64) -- (494.68,71)  ;
%Shape: Right Triangle [id:dp441461564376495] 
\draw  [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=0.25 ] (489,95) -- (610.8,196.36) -- (489,196.36) -- cycle ;
%Curve Lines [id:da691862389693042] 
\draw [line width=0.75]    (590.8,116.16) .. controls (573.16,147.52) and (568.97,116.46) .. (549.04,139.67) ;
\draw [shift={(547.8,141.16)}, rotate = 308.93] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-4.9) .. controls (6.95,-2.3) and (3.31,-0.67) .. (0,0) .. controls (3.31,0.67) and (6.95,2.3) .. (10.93,4.9)   ;
%Shape: Rectangle [id:dp29784833864235405] 
\draw  [color={rgb, 255:red, 95; green, 19; blue, 254 }  ,draw opacity=0.23 ][fill={rgb, 255:red, 95; green, 19; blue, 254 }  ,fill opacity=0.23 ] (120.8,155.16) -- (260.8,155.16) -- (260.8,216.36) -- (120.8,216.36) -- cycle ;
%Straight Lines [id:da014819478856842094] 
\draw [line width=1.5]    (81.8,55.36) -- (260.8,55.36) ;
%Straight Lines [id:da19136676020039034] 
\draw [line width=1.5]    (80.8,115.36) -- (260.8,116.36) ;
%Straight Lines [id:da019274737615810222] 
\draw    (61.8,85.36) -- (89.8,85.36) ;
\draw [shift={(91.8,85.36)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da43759945225025065] 
\draw [line width=1.5]    (260.8,55.36) -- (260.8,116.36) ;
%Shape: Rectangle [id:dp8414125012045715] 
\draw  [color={rgb, 255:red, 95; green, 19; blue, 254 }  ,draw opacity=0.23 ][fill={rgb, 255:red, 95; green, 19; blue, 254 }  ,fill opacity=0.23 ] (180.8,55.16) -- (260.8,55.16) -- (260.8,116.36) -- (180.8,116.36) -- cycle ;

% Text Node
\draw (8,176) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle A_{2}( t)$};
% Text Node
\draw (7,76) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle A_{1}( t)$};
% Text Node
\draw (206,12) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle Q_{1}( t)$};
% Text Node
\draw (167,241) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle Q_{2}( t)$};
% Text Node
\draw (361,100.4) node [anchor=north west][inner sep=0.75pt]    {$\mathbf{D}( t)$};
% Text Node
\draw (457,65.4) node [anchor=north west][inner sep=0.75pt]  [font=\large]  {$\lambda _{2}$};
% Text Node
\draw (623,196.4) node [anchor=north west][inner sep=0.75pt]  [font=\large]  {$\lambda _{1}$};
% Text Node
\draw (567,94.4) node [anchor=north west][inner sep=0.75pt]  [font=\normalsize]  {$\lambda _{1} +\lambda _{2} =1$};


\end{tikzpicture}

% \begin{tikzpicture}[x=0.5pt,y=0.5pt,yscale=-1,xscale=1]
% %uncomment if require: \path (0,240); %set diagram left start at 0, and has height of 240

% %Straight Lines [id:da09715700995858345] 
% \draw    (85.8,140.36) -- (264.8,139.36) ;
% %Straight Lines [id:da8887479227991981] 
% \draw    (85.8,198.36) -- (265.8,199.36) ;
% %Straight Lines [id:da8614120669050047] 
% \draw    (264.8,139.36) -- (265.8,199.36) ;
% %Straight Lines [id:da6217209993953612] 
% \draw    (54.8,169.36) -- (82.8,169.36) ;
% \draw [shift={(84.8,169.36)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
% %Straight Lines [id:da4398173253440574] 
% \draw    (84.8,40.36) -- (263.8,39.36) ;
% %Straight Lines [id:da5015891688166809] 
% \draw    (84.8,98.36) -- (264.8,99.36) ;
% %Straight Lines [id:da875509031522369] 
% \draw    (263.8,39.36) -- (264.8,99.36) ;
% %Straight Lines [id:da6528587077790915] 
% \draw    (53.8,69.36) -- (81.8,69.36) ;
% \draw [shift={(83.8,69.36)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
% %Rounded Rect [id:dp4517176185326244] 
% \draw  [color={rgb, 255:red, 81; green, 74; blue, 226 }  ,draw opacity=1 ][fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ] (156.8,53.67) .. controls (156.8,47.78) and (161.58,43) .. (167.47,43) -- (250.33,43) .. controls (256.22,43) and (261,47.78) .. (261,53.67) -- (261,85.69) .. controls (261,91.58) and (256.22,96.36) .. (250.33,96.36) -- (167.47,96.36) .. controls (161.58,96.36) and (156.8,91.58) .. (156.8,85.69) -- cycle ;
% %Rounded Rect [id:dp225981923335425] 
% \draw  [color={rgb, 255:red, 81; green, 74; blue, 226 }  ,draw opacity=1 ][fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ] (105.8,153.67) .. controls (105.8,147.78) and (110.58,143) .. (116.47,143) -- (252.33,143) .. controls (258.22,143) and (263,147.78) .. (263,153.67) -- (263,185.69) .. controls (263,191.58) and (258.22,196.36) .. (252.33,196.36) -- (116.47,196.36) .. controls (110.58,196.36) and (105.8,191.58) .. (105.8,185.69) -- cycle ;
% %Straight Lines [id:da37671038244024846] 
% \draw    (156,29) -- (260.8,29) ;
% \draw [shift={(263.8,29)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
% \draw [shift={(153,29)}, rotate = 0] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
% %Straight Lines [id:da0678614898035077] 
% \draw    (111.8,209) -- (263.8,209) ;
% \draw [shift={(266.8,209)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
% \draw [shift={(108.8,209)}, rotate = 0] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
% %Shape: Circle [id:dp028275738414681006] 
% \draw  [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=0.67 ] (365,126.18) .. controls (365,118) and (371.63,111.36) .. (379.82,111.36) .. controls (388,111.36) and (394.64,118) .. (394.64,126.18) .. controls (394.64,134.37) and (388,141) .. (379.82,141) .. controls (371.63,141) and (365,134.37) .. (365,126.18) -- cycle ;
% %Curve Lines [id:da7202837492936005] 
% \draw    (343.8,61.36) .. controls (279.45,106.9) and (302.33,157.34) .. (342.58,188.43) ;
% \draw [shift={(343.8,189.36)}, rotate = 217.09] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
% %Straight Lines [id:da4678251099443136] 
% \draw    (365,126.18) -- (288.45,73.5) ;
% \draw [shift={(286.8,72.36)}, rotate = 394.53999999999996] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
% %Shape: Axis 2D [id:dp8494447421977243] 
% \draw [line width=1.5]  (461,179.73) -- (637.8,179.73)(478.68,48) -- (478.68,194.36) (630.8,174.73) -- (637.8,179.73) -- (630.8,184.73) (473.68,55) -- (478.68,48) -- (483.68,55)  ;
% %Shape: Right Triangle [id:dp441461564376495] 
% \draw  [fill={rgb, 255:red, 74; green, 120; blue, 226 }  ,fill opacity=0.6 ] (478,79) -- (599.8,180.36) -- (478,180.36) -- cycle ;
% %Curve Lines [id:da691862389693042] 
% \draw [line width=0.75]    (579.8,100.16) .. controls (562.16,131.52) and (557.97,100.46) .. (538.04,123.67) ;
% \draw [shift={(536.8,125.16)}, rotate = 308.93] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-4.9) .. controls (6.95,-2.3) and (3.31,-0.67) .. (0,0) .. controls (3.31,0.67) and (6.95,2.3) .. (10.93,4.9)   ;

% % Text Node
% \draw (8,160) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle A_{2}( t)$};
% % Text Node
% \draw (7,60) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle A_{1}( t)$};
% % Text Node
% \draw (186,5) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle Q_{1}( t)$};
% % Text Node
% \draw (169,213) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle Q_{2}( t)$};
% % Text Node
% \draw (361,88.4) node [anchor=north west][inner sep=0.75pt]    {$\mathbf{D}( t)$};
% % Text Node
% \draw (446,49.4) node [anchor=north west][inner sep=0.75pt]  [font=\large]  {$\lambda _{2}$};
% % Text Node
% \draw (612,180.4) node [anchor=north west][inner sep=0.75pt]  [font=\large]  {$\lambda _{1}$};
% % Text Node
% \draw    (526,68) -- (635,68) -- (635,99) -- (526,99) -- cycle  ;
% \draw (529,72.4) node [anchor=north west][inner sep=0.75pt]  [font=\large]  {$\lambda _{1} +\lambda _{2} \leq 1$};
% % Text Node
% \draw (461,175.4) node [anchor=north west][inner sep=0.75pt]  [font=\Large]  {$o$};


%\end{tikzpicture}
}

==> mainresults.tex <==
\setlength{\textfloatsep}{10pt}
\subsection{Finite State - Action MDPs}
In this section, we describe the convergence rate of the softmax policy gradient Algorithm ~\ref{alg:mainPolicyGradMDP} for finite SA MDPs. The following result shows that the value function converges to the value function of the \emph{best in-class} policy at a rate $\cO\left(\frac{1}{t}\right)$. Furthermore, the theorem shows an explicit dependence on the number of controllers $M$. 

\textbf{Technical Novelty.} We note here that while the basic recipe for the analysis of Theorem \ref{thm:convergence of policy gradient} is similar to \cite{Mei2020}, we stress that our setting does not directly inherit the intuition of standard PG analysis (sPG). %\avim{ because our controller interacts with the system only through the available policies and }
(1) With $|\mathcal{S}\times\mathcal{A}|<\infty,$ the sPG analysis critically depends on the fact that a  deterministic optimal policy exists and shows convergence to it. Our setting enjoys no such guarantee.
(2) The value function gradient in sPG has no `cross contamination' from other states, so modifying the parameter of one state does not affect the values of the others. Our setting cannot leverage this since the value function gradient possesses contributions from \emph{all} states (see Lemma \ref{lemma:Gradient simplification}). Hence, our analysis becomes more intricate than existing techniques or simple modifications thereof.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{theorem}
% The policy gradient rule stated  in Algorithm \ref{alg:mainPolicyGradMDP} guarantees that there exists $V^\infty(s)$ and $\Q^\infty(s,m)$, for all states $s\in \cS$, and for all $m\in [M]$, such that $V^{(t)}(s)\to V^\infty(s)$ and $\Q^{(t)}(s,m)\to \Q^\infty(s,m)$.
% \end{theorem}
%\avim{mention that $S\geq2$ here.} 

\begin{restatable}[Convergence of Policy Gradient]{theorem}{maintheorem}\label{thm:convergence of policy gradient}
%Assumption \ref{assumption:positivity of advantage} and \ref{assumption:positive c}, and 
With $\{\theta_t \}_{t\geq 1}$ generated as in Algorithm \ref{alg:mainPolicyGradMDP} and using a learning rate $\eta = \frac{\left(1-\gamma\right)^2}{7\gamma^2+4\gamma+5}$, for all $t\geq 1$,
% \[V^*(\rho) -V^{\pi_{\theta_t}}(\rho) \leq {\color{blue}\frac{1}{t}} M \left(\frac{7\gamma^2+4\gamma+5}{c^2(1-\gamma)^3}\right)\norm{\frac{d_\mu^{\pi^*}}{\mu}}_{\infty}^2 \norm{\frac{1}{\mu}}_\infty.  \]
\begin{equation}\label{eqn:PGConvergeFiniteMDPs}
    V^*(\rho) -V^{\pi_{\theta_t}}(\rho) \leq {\color{blue}\frac{1}{t}} M \left(\frac{7\gamma^2+4\gamma+5}{c^2(1-\gamma)^3}\right)\norm{\frac{d_\mu^{\pi^*}}{\mu}}_{\infty}^2 \norm{\frac{1}{\mu}}_\infty. 
\end{equation}
\end{restatable}
%\vspace{-0.3cm}
\begin{remark}
The quantity $c$ in the statement is the minimum probability that SoftMax PG puts on the controllers for which the best mixture $\pi^*$ puts positive probability mass. While we currently do not supply a lower bound for $c,$ empirical studies presented in Sec.~\ref{sec:simulation-results} clearly show that $c$ is indeed lower bounded, rendering the bound in \eqref{eqn:PGConvergeFiniteMDPs} non vacuous.
\end{remark}
\ag{Please define $c$ mathematically and mention in the figure caption}

%\vspace{-0.5cm}
\begin{proof}[Proof sketch of Theorem \ref{thm:convergence of policy gradient}] We highlight here the main steps of the proof. We begin by showing that in our case the gradient of $V^{\pi_\theta}(\mu)$ can be simplified as follows.
\begin{restatable}[Gradient Simplification]{lemma}{gradientofV}\label{lemma:Gradient simplification}
The softmax policy gradient with respect to the parameter $\theta\in \Real^M$ is
\[\frac{\partial}{\partial \theta_m}V^{\pi_{\theta}}(\mu) = \frac{1}{1-\gamma}\sum\limits_{s\in \cS}d_\mu^{\pi_\theta}(s) \pi_\theta(m)\tilde{A}(s,m). \]
where $\tilde{A}(s,m):=\Q(s,m)-V(s)$ and $\Q(s,m):= \sum\limits_{a\in \cA}K_m(s,a)Q^{\pi_\theta}(s,a) $, and $d_\mu^{\pi_\theta}(.)$ is the \textit{discounted state visitation measure} starting with an initial distribution $\mu$ and following policy $\pi_\theta$.
\end{restatable}
%\vspace{-0.3cm}
The interpretation here being $\tilde{A}(s,m)$ is the advantage of following controller $m$ at state $s$ and then following the policy $\pi_\theta$ for all time versus following $\pi_\theta$ always.
As mentioned in section \ref{sec:bandit over bandit}, we proceed by proving smoothness of $V$ function over the space $\Real^M$.
%[Smoothness of ${V}^{\pi_{\theta}}\left(\mu\right)$]
\begin{restatable} {lemma}{smoothnesslemmaMDP}\label{lemma:smoothness of V}
${V}^{\pi_{\theta}}\left(\mu\right)$ is $\frac{7\gamma^2+4\gamma+5}{2\left(1-\gamma\right)^2}$-smooth.
\end{restatable}
%\vspace{-0.3cm}
Next we show a novel {\L}ojaseiwicz type inequality which lower bounds the magnitude of the gradient of the value function.
%\vspace{-0.15cm}
\begin{restatable}[Non-uniform {\L}ojaseiwicz inequality]{lemma}{nonuniformLE}\label{lemma:nonuniform lojaseiwicz inequality}
\begin{equation*}
\norm{\frac{\partial}{\partial\theta}V^{\pi_\theta}(\mu)}_2 \geq \frac{1}{\sqrt{M}}\left(\min\limits_{m:\pi^*_{\theta_{m}}>0} \pi_{\theta_m} \right) \times \norm{\frac{d_{\rho}^{\pi^*}}{d_{\mu}^{\pi_\theta}}}_{\infty}^{-1} \left[V^*(\rho) -V^{\pi_\theta}(\rho) \right]. 
\end{equation*}
\end{restatable}
The rest of the proof follows by combining Lemmas \ref{lemma:Gradient simplification}, \ref{lemma:smoothness of V} and \ref{lemma:nonuniform lojaseiwicz inequality} followed by an induction argument over $t\geq 1$.
\end{proof}
%\vspace{-1cm}
Having provided performance guarantees for our algorithms for both MABs and finite MDPs, we now move on to experimental results.
